Knowledge-based Emotion Recognition using Large Language Models

Emotion recognition in social situations is a complex task that requires integrating information from both facial expressions and the situational context. While traditional approaches to automatic emotion recognition have focused on decontextualized signals, recent research emphasizes the importance of context in shaping emotion perceptions. This paper contributes to the emerging field of context-based emotion recognition by leveraging psychological theories of human emotion perception to inform the design of automated methods. We propose an approach that combines emotion recognition methods with Bayesian Cue Integration (BCI) to integrate emotion inferences from decontextualized facial expressions and contextual knowledge inferred via Large-language Models. We test this approach in the context of interpreting facial expressions during a social task, the prisoner's dilemma. Our results provide clear support for BCI across a range of automatic emotion recognition methods. The best automated method achieved results comparable to human observers, suggesting the potential for this approach to advance the field of affective computing.

==> Sections/02_Data.tex <==
\section{EMOTION PERCEPTION RATINGS}

To examine how context and expression interact to shape emotion perception, we requested archival video data
of people engaged in a social task and asked multiple raters to separately annotate the perceived emotion of the person in the video (some with and some without context).

\subsection{Archival Data}

We requested archival data from the University of Southern California’s Split-Steal dataset. This is a large collection of participants that engaged in an iterated prisoner’s dilemma task as described in~\cite{lei2023emotional}. Participants could see each other but not speak and were incentivized by playing for lottery tickets for several \$100 USD lotteries. The dataset consists of 7 second “reaction shots” when players learn of their joint choice on a given round in the prisoner’s  dilemma. 
%These videos have been automatically rated for facial action units using a commercial tool based on CERT~\cite{littlewort2011computer} and automatically rated for facial expressivity using the method proposed in~\cite{lei2023emotional}.

In the prisoner’s dilemma, players separately decided whether to try and split or steal a pot of lottery tickets on each round of the game. 
They receive lottery tickets based  on their joint action. If both choose split (designated CC for mutual cooperation), they split ten tickets. 
If Player A chooses split and Player B chooses steal (designated CD for cooperate-defect), then Player B receives all the tickets and Player A receives none. If they both steal (designated DD), each player receives a single ticket.
In the prisoner’s dilemma, players separately decided whether to try and split or steal a pot of lottery tickets on each round of the game. 
They receive lottery tickets based on their joint action. If both choose split (designated CC for mutual cooperation), they split ten tickets. If Player A chooses split and Player B chooses steal (designated CD for cooperate-defect), then Player B receives all the tickets and Player A receives none. 
If they both steal (designated DD), each player receives a single ticket.
As our interest was examining perception of emotion, rather than predicting self-reported feelings or game outcomes, we selected a subset of highly expressive videos from the archive. 
Specifically, we chose 25 of the most expressive videos for each possible outcome in the game. 
Expressivity was determined using the automatic labels provided with each video (no human judgment was used to select these videos). 
This resulted in a database of 100 7-second video clips, 25 from each of the four actual game outcomes: CC, CD, DC, and DD.

\subsection{Perception Ratings from Face and Context}

We recruited a sample of annotators through Amazon Mechanical Turk to provide emotion perception ratings of the videos. 
For each video, annotators were asked Basic emotion label (\textit{``Which of the following words best describes the facial expression (choosing from anger, disgust, fear, joy, sadness, surprise or neutral)"})

The annotation task was performed by manipulating context in two ways. Each annotator rated 10 randomly selected videos and twenty ratings were obtained for each video in each context. 
The contexts are illustrated in Fig.~\ref{fig:context_level}.

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{Figures/Facial_Annotation.jpg}
    \caption{Facial reactions were annotated either without context (zero context), with instruction about the joint outcome of the game (in this case mutual cooperation) seeing the reaction of both players reactions (w/ context). }
    \label{fig:context_level}
\end{figure}

\textbf{Zero-context}: %(henceforth called “w/o”)}: 
Annotators were asked to answer the above questions only by seeing the video of one player. They were not told this was from a game but just told to watch the video and answer the questions. They were free to watch the video as many times as possible.

\textbf{With context}:  Annotators first read a description of the prisoner’s dilemma task, including the payoff for different joint decisions.  Following this, they were quizzed on details of the game and annotators were excluded from the task if their answers were incorrect.
If annotators successfully displayed an understanding of the game, they were then shown a sequence of videos drawn from the actual joint outcome of the round. 
For each video, they were provided the joint outcome and told to rate the reaction of the player in the red box and were free to watch the video as many times as possible.


\subsection{Emotion Probability Distribution}
%Can you point me to prior papers that recognize a distribution of emotion
In our paper, we have chosen to frame the task as a probability distribution regression problem, drawing inspiration from the challenges of subjective perception in image emotion recognition (IER) highlighted by Zhao et al.~\cite{zhao2017approximating} and others. 
The inherent subjectivity of emotions, influenced by factors such as cultural background, personality, and social context, leads to inconsistent labeling of emotions in images~\cite{joshi2011aesthetics,zhao2014exploring,peng2015mixed }. 
This variability is exemplified by the fact that images within the same discrete emotion category can exhibit significant differences in emotion variance among viewers.
Our approach aims to capture the full spectrum of emotion. 
By modeling emotion as a probability distribution, we can provide a more comprehensive and accurate representation of the emotional content in images,accounting for the diverse and subjective nature of human emotion perception.


